From Plan to Action: How Well Do Agents Follow the Plan?

Agents are commonly instructed to follow a task-specific plan for guidance. However, it is unknown to what extent agents actually follow instructed plans. Without such an analysis, determining the extent agents comply with a given plan, it is impossible to assess whether a solution was reached through correct strategic reasoning or through other means, e.g., data contamination or overfitting to a benchmark. This paper presents the first extensive, systematic analysis of plan compliance in programming agents, examining 21,120 trajectories from SWE-agent across four LLMs on SWE-bench Verified and SWE-bench Pro under eight plan variations. Without an explicit plan, agents fall back on internalized workflows during training, which are often incomplete, overfit, or inconsistently applied. Providing the standard plan improves issue resolution, and we observe that periodic plan reminders can mitigate plan violations and improve task success. A subpar plan hurts performance even more than no plan at all. Surprisingly, inserting additional task-relevant phases in the early stage can degrade performance, particularly when these phases do not align with the model's internal problem-solving strategy. These findings call for fine-tuning paradigms that teach models to follow instructed plans, rather than encoding task-specific plans in them, so that they reason and act adaptively, rather than memorizing workflows.

==> figures/no_plan/no_plan_heatmap_compliance.tex <==
\begin{figure}[htb]
% \begin{wrapfigure}{r}{0.49\textwidth}
\centering
\includegraphics[width=0.99\linewidth]{figures/no_plan/no_plan_heatmap_compliance.png}
\caption{No plan different settings Model Compliance Comparison: Resolved vs.\ Unresolved Issues.}
% add a pargraph discussing what new vocabularies are added per each model (vocab). can refer to sankey
% % add a pargraph discussing what vocabularies are missing (coverage). can refer to sankey

\label{fig:noplan_compliance_heatmap}
\end{figure}
% \end{wrapfigure}

==> figures/no_plan/no_plan_trajectory_analysis.tex <==
% \begin{figure}[t]
\begin{wrapfigure}{r}{0.49\textwidth}
\centering
\includegraphics[width=0.99\linewidth]{figures/no_plan/no_plan_trajectory_analysis.png}
\caption{Comparison of trajectories different models}
\label{fig:noplan_traj}
% \vspace{-1pt}
% \end{figure}
\end{wrapfigure}

==> figures/no_plan/no_plan_vs_plan_success.tex <==
\begin{figure}[htb]
% \begin{wrapfigure}{r}{0.49\textwidth}
\centering
\includegraphics[width=0.99\linewidth]{figures/no_plan/no_plan_vs_plan_success.png}
\caption{Comparison of success rate plan vs no\_plan settings}
\label{fig:noplan_success}
% \vspace{-1pt}
\end{figure}
% \end{wrapfigure}

==> figures/no_plan/no_plan_vs_plan_success_and_traj.tex <==
\begin{figure}[htb]
% \begin{wrapfigure}{r}{0.49\textwidth}
\centering
\includegraphics[width=0.99\linewidth]{figures/no_plan/no_plan_vs_plan_success_and_traj.png}
\textcolor{blue}{MH: the fonts in this figure are too tiny.}
\caption{Comparison of success rate and trajectories in  plan vs no\_plan settings}
\label{fig:noplan_traj_success}
% \vspace{-1pt}
\end{figure}
% \end{wrapfigure}

==> figures/no_plan/no_plan_vs_plan_trajectory_comp.tex <==
\begin{figure}[htb]
% \begin{wrapfigure}{r}{0.49\textwidth}
\centering
\includegraphics[width=0.99\linewidth]{figures/no_plan/no_plan_vs_plan_trajectory_comp.png}
\caption{Comparison of trajectories plan vs no\_plan settings}
\label{fig:noplan_traj}
% \vspace{-1pt}
\end{figure}
% \end{wrapfigure}

==> figures/plan/plan_comp_heatmap.tex <==
\begin{figure}[htb]
% \begin{wrapfigure}{r}{0.49\textwidth}
\centering
\includegraphics[width=0.99\linewidth]{figures/plan/plan_comp_heatmap.png}
\caption{Model Compliance Comparison: Resolved vs.\ Unresolved Issues. \jatin{IMO too many numbers and we should merge Resolved+Unresolved categories into a single overall score at this point in the paper. We should move the current plot to Appendix and have a short para over it further.}}
% add a pargraph discussing what new vocabularies are added per each model (vocab). can refer to sankey
% % add a pargraph discussing what vocabularies are missing (coverage). can refer to sankey

\label{fig:compliance-heatmap}
\end{figure}
% \end{wrapfigure}

==> figures/plan/plan_trajectory_analysis.tex <==
\begin{figure}[htb]
% \begin{wrapfigure}{r}{0.49\textwidth}
\centering
\includegraphics[width=0.99\linewidth]{figures/plan/plan_trajectory_analysis.png}
\caption{Comparison of trajectories different models in default plan settings}
\label{fig:plan_traj}
% \vspace{-1pt}
\end{figure}
% \end{wrapfigure}

==> figures/plan/plan_venn.tex <==
\begin{figure}[htb]
% \begin{wrapfigure}{r}{0.49\textwidth}
\centering
\includegraphics[width=0.8\linewidth]{figures/plan/plan_venn.png}
\vspace{-14pt}
\caption{Instances overlap across different models}
\label{fig:plan_venn}
% \vspace{-1pt}
\end{figure}
% \end{wrapfigure}

==> figures/step_added/heatmap_added_step.tex <==
\begin{figure}[htb]
% \begin{wrapfigure}{r}{0.49\textwidth}
\centering
\includegraphics[width=0.99\linewidth]{figures/step_added/heatmap_added_step.png}
\caption{Compliance rate step added, reordered, and reminded}
\label{fig:addsteps_heatmap}
% \vspace{-1pt}
\end{figure}
% \end{wrapfigure}

==> figures/step_added/merged_step_add_success_and_traj.tex <==
\begin{figure}[htb]
% \begin{wrapfigure}{r}{0.49\textwidth}
\centering
\includegraphics[width=0.99\linewidth]{figures/step_added/merged_step_add_success_and_traj.png}
\caption{step added success rate and trajectory analysis}
\label{fig:addsteps_success_and_traj}
% \vspace{-1pt}
\end{figure}
% \end{wrapfigure}

==> figures/step_added/reminded_sankey.tex <==
\begin{figure*}[t]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{5pt} % horizontal spacing between images
    \renewcommand{\arraystretch}{1.35}
    
    % \begin{tabular}{ccc}
    \begin{tabular}{cccc}
         \footnotesize
         
        \includegraphics[width=0.23\textwidth]{figures/step_added/reminded/sa_dev_sankey.pdf} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/reminded/sa_gpt5m_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/step_added/reminded/sa_dsk-v3_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/step_added/reminded/sa_dsk-r1_sankey.pdf} \\[6pt]

        Devstral-small & GPT5-mini & DeepSeek-V3 & DeepSeek-R1 \\
    \end{tabular}
    \vspace{-8pt}
    \caption{Phase flow analysis under Plan reminded setting, with respect to the Standard Plan phases ($\mathcal{L}^\star(\Phi)=(\colorbox[HTML]{CCC7E6}{N}\colorbox[HTML]{EEC7D4}{R}\colorbox[HTML]{FFED99}{P}\colorbox[HTML]{D9EDCC}{V})$).}
    \label{fig:sankey-reminded}
\end{figure*}

==> figures/step_added/sankey.tex <==
\begin{figure*}[htbp]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{5pt} % horizontal spacing between images
    \renewcommand{\arraystretch}{1.35}
    
    % \begin{tabular}{ccc}
    \begin{tabular}{@{}l@{\quad}cccc@{}}
         \footnotesize
        % \toprule
        & regression & summary & reordered & reminded \\
        % \midrule

        % \textbf{Devstral} &
         \rotatebox{90}{\centering Devstral} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/regression/sa_dev_sankey.pdf} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/summary/sa_dev_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/step_added/reordered/sa_dev_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/step_added/reminded/sa_dev_sankey.pdf} \\[6pt]
        
        \rotatebox{90}{\centering GPT5-mini} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/regression/sa_gpt5m_sankey.pdf} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/summary/sa_gpt5m_sankey.pdf} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/reordered/sa_gpt5m_sankey.pdf} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/reminded/sa_gpt5m_sankey.pdf}\\[6pt]

        \rotatebox{90}{\centering Deepseek-V3} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/regression/sa_dsk-v3_sankey.pdf} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/summary/sa_dsk-v3_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/step_added/reordered/sa_dsk-v3_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/step_added/reminded/sa_dsk-v3_sankey.pdf} \\[6pt]
        
        \rotatebox{90}{\centering Deepseek-R1} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/regression/sa_dsk-r1_sankey.pdf} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/summary/sa_dsk-r1_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/step_added/reordered/sa_dsk-r1_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/step_added/reminded/sa_dsk-r1_sankey.pdf} \\[6pt]




    \end{tabular}

    \caption{Phase transition sequences (cut-off = 10) in step added settings}
    \label{fig:addsteps_sankey}
\end{figure*}

==> figures/step_added/summary_sankey.tex <==
\begin{figure*}[t]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{5pt} % horizontal spacing between images
    \renewcommand{\arraystretch}{1.35}
    
    % \begin{tabular}{ccc}
    \begin{tabular}{cccc}
         \footnotesize
         
        \includegraphics[width=0.23\textwidth]{figures/step_added/summary/sa_dev_sankey.pdf} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/summary/sa_gpt5m_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/step_added/summary/sa_dsk-v3_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/step_added/summary/sa_dsk-r1_sankey.pdf} \\[6pt]

        Devstral-small & GPT5-mini & DeepSeek-V3 & DeepSeek-R1 \\
    \end{tabular}
    \vspace{-8pt}
    \caption{Phase flow analysis under Regression Testing () and Summary plan setting ().}
    \label{fig:sankey-summary}
\end{figure*}

==> figures/step_removal/heatmap_removal_step.tex <==
\begin{figure}[htb]
% \begin{wrapfigure}{r}{0.49\textwidth}
\centering
\includegraphics[width=0.99\linewidth]{figures/step_removal/heatmap_removal_step.png}
\caption{Compliance rate step removal \jatin{Very small font.}}
\label{fig:removesteps_heatmap}
% \vspace{-1pt}
\end{figure}
% \end{wrapfigure}

==> figures/step_removal/merged_step_removal_success_and_traj.tex <==
\begin{figure}[htb]
% \begin{wrapfigure}{r}{0.49\textwidth}
\centering
\includegraphics[width=0.99\linewidth]{figures/step_removal/merged_step_removal_success_and_traj.png}
\caption{step removal success rate and trajectory analysis}
\label{fig:removesteps_success_and_traj}
% \vspace{-1pt}
\end{figure}
% \end{wrapfigure}

==> figures/step_removal/no_validation_sankey.tex <==
\begin{figure*}[t]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{5pt} % horizontal spacing between images
    \renewcommand{\arraystretch}{1.35}
    
    % \begin{tabular}{ccc}
    \begin{tabular}{cccc}
         \footnotesize
         
        \includegraphics[width=0.23\textwidth]{figures/step_removal/no_verif/sa_dev_sankey.pdf} & 
        \includegraphics[width=0.23\textwidth]{figures/step_removal/no_verif/sa_gpt5m_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/step_removal/no_verif/sa_dsk-v3_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/step_removal/no_verif/sa_dsk-r1_sankey.pdf} \\[6pt]

        Devstral-small & GPT5-mini & DeepSeek-V3 & DeepSeek-R1 \\
    \end{tabular}
    \vspace{-8pt}
    \caption{Phase flow analysis under No Validation plan setting ($\mathcal{L}^\star(\Phi)=(\colorbox[HTML]{CCC7E6}{N},\colorbox[HTML]{EEC7D4}{R},\colorbox[HTML]{FFED99}{P})$).}
    \label{fig:sankey-no-validation}
\end{figure*}

==> figures/step_removal/sankey.tex <==
\begin{figure*}[t]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{5pt} % horizontal spacing between images
    \renewcommand{\arraystretch}{1.35}
    
    \begin{tabular}{@{}l@{\quad}cccc@{}}
         \footnotesize
        \vspace{-0.2cm}
         \rotatebox{90}{
  \begin{minipage}{1.5cm} % Adjust this width to match your cell height
    \centering Reordered
  \end{minipage}
} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/reordered/sa_dev_sankey.pdf} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/reordered/sa_gpt5m_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/plan/sa_dsk-v3_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/step_added/reordered/sa_dsk-r1_sankey.pdf} \\[6pt]
        \vspace{-0.2cm}
        \rotatebox{90}{
  \begin{minipage}{1.5cm} % Adjust this width to match your cell height
    \centering Regression
  \end{minipage}
} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/regression/sa_dev_sankey.pdf} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/regression/sa_gpt5m_sankey.pdf} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/regression/sa_dsk-v3_sankey.pdf} & 
        \includegraphics[width=0.23\textwidth]{figures/step_added/regression/sa_dsk-r1_sankey.pdf}\\[6pt]
        \vspace{-0.2cm}
        \rotatebox{90}{
  \begin{minipage}{1.5cm} % Adjust this width to match your cell height
    \centering No Validation
  \end{minipage}
} & 
        \includegraphics[width=0.23\textwidth]{figures/step_removal/no_verif/sa_dev_sankey.pdf} & 
        \includegraphics[width=0.23\textwidth]{figures/step_removal/no_verif/sa_gpt5m_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/step_removal/no_verif/sa_dsk-v3_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/step_removal/no_verif/sa_dsk-r1_sankey.pdf} \\[6pt]
        \vspace{-0.2cm}
        \rotatebox{90}{
  \begin{minipage}{1.5cm} % Adjust this width to match your cell height
    \centering No Reproduce
  \end{minipage}
} & 
        \includegraphics[width=0.23\textwidth]{figures/step_removal/no_reproduce/sa_dev_sankey.pdf} & 
        \includegraphics[width=0.23\textwidth]{figures/step_removal/no_reproduce/sa_gpt5m_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/step_removal/no_reproduce/sa_dsk-v3_sankey.pdf} &
        \includegraphics[width=0.23\textwidth]{figures/step_removal/no_reproduce/sa_dsk-r1_sankey.pdf} \\[6pt]

        & Devstral-small & GPT5-mini & DeepSeek-V3 & DeepSeek-R1 \\
        
    \end{tabular}

    \caption{Phase flow analysis trajectories under mutated plan setting ($\mathcal{L}^\star(\Phi)=(\colorbox[HTML]{CCC7E6}{N}\colorbox[HTML]{EEC7D4}{R}\colorbox[HTML]{FFED99}{P}\colorbox[HTML]{D9EDCC}{V})$). Flow thickness is the number trajectories transitions from one phase to another. The black bar indicates trajectory termination.  
    }
    \label{fig:mutate-compliance-sankey}
\end{figure*}

==> figures/step_removal/step_removal_success.tex <==
\begin{figure}[htb]
% \begin{wrapfigure}{r}{0.49\textwidth}
\centering
\includegraphics[width=0.99\linewidth]{figures/step_removal/step_removal_success.png}
\caption{step removal success rate and trajectories analysis}
\label{fig:removesteps_success}
% \vspace{-1pt}
\end{figure}
% \end{wrapfigure}

==> figures/step_removal/traj_analysis_remove_steps.tex <==
\begin{figure}[htb]
% \begin{wrapfigure}{r}{0.49\textwidth}
\centering
\includegraphics[width=0.99\linewidth]{figures/step_removal/traj_analysis_remove_steps.png}
\caption{Comparison of trajectories steps removal settings}
\label{fig:removesteps_traj}
% \vspace{-1pt}
\end{figure}
% \end{wrapfigure}

==> tables/no_plan_lcp.tex <==
\makeatletter
\newcommand{\pat}[1]{%
  \begingroup\mathsurround=0pt
  \catcode`\,=\active \catcode`\(=\active \catcode`\)=\active
  \def,{\mskip\thinmuskip\allowbreak,\mskip\thinmuskip}%
  \def({\mskip\thinmuskip(\allowbreak}%
  \def){\allowbreak)\mskip\thinmuskip}%
  \ensuremath{\langle #1 \rangle}%
  \endgroup
}
\makeatother
% Compact but readable table spacing
\newcolumntype{Z}{>{\raggedright\arraybackslash}X}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.06}

\begin{table*}[t]
\centering
\footnotesize
\caption{No plan settings. Top $\mathcal{LCP}$s of studied models, conditioned on repair status and problem difficulty. Superscripts denote pattern repetition and subscripts denote phase duration (run-length from \lang).}
% %\vspace{-10pt}
\label{tab:noplan_lcp}
\begin{tabularx}{\textwidth}{l @{\extracolsep{\fill}} ccc ccc }
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Resolved}} & \multicolumn{3}{c}{\textbf{Unresolved}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& easy & medium & hard & easy & medium & hard \\
\midrule
Devstral & (N, R)^3 & (N, R)^3 & (N, R)^4 & (N, R)^3 & (N, R)^4 & (N, R)^3 \\
GPT5-mini & (N, P)^3 & (N, P)^3 & (N_3, P)^2, N, V & (N, P)^3 & (N, P)^3, V & (N, P)^5 \\
Deepseek-V3 & N, P & N, P & P & N, P & N, P & N, P \\
Deepseek-R1 & N, P & N, P & P & N, P & N, P, N & N, P \\
\bottomrule
\end{tabularx}
\label{tab:noplan_lcp}
\end{table*}

==> tables/plan_compliance_rate.tex <==
\begin{table}[htbp]
\centering
\footnotesize
\caption{Model Compliance Comparison: Resolved vs. Unresolved Issues}
\label{tab:plan_compliance}
\begin{tabularx}{\textwidth}{l @{\extracolsep{\fill}} ccc ccc c}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Resolved}} & \multicolumn{3}{c}{\textbf{Unresolved}} & \textbf{Overall} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& Vocab & Cov. & Order & Vocab & Cov. & Order & \textbf{Score} \\
\midrule
GPT5-mini & 0.82 & 0.72 & 0.72 & 0.82 & 0.76 & 0.76 & 0.76 \\
Deepseek-V3 & 0.99 & 0.79 & 0.74 & 0.99 & 0.77 & 0.73 & 0.82 \\
Devstral-small & 0.8 & 0.99 & 0.99 & 0.81 & 0.95 & 0.95 & 0.91 \\
Deepseek-R1 & 0.86 & 0.73 & 0.69 & 0.87 & 0.68 & 0.63 & 0.73 \\
\bottomrule
\end{tabularx}
\end{table}

==> tables/plan_lcp.tex <==
\makeatletter
\newcommand{\pat}[1]{%
  \begingroup\mathsurround=0pt
  \catcode`\,=\active \catcode`\(=\active \catcode`\)=\active
  \def,{\mskip\thinmuskip\allowbreak,\mskip\thinmuskip}%
  \def({\mskip\thinmuskip(\allowbreak}%
  \def){\allowbreak)\mskip\thinmuskip}%
  \ensuremath{\langle #1 \rangle}%
  \endgroup
}
\makeatother
% Compact but readable table spacing
\newcolumntype{Z}{>{\raggedright\arraybackslash}X}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.06}

\begin{table*}[t]
\centering
\footnotesize
% %\vspace{-10pt}
\begin{tabularx}{\textwidth}{l @{\extracolsep{\fill}} ccc ccc }
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Resolved}} & \multicolumn{3}{c}{\textbf{Unresolved}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& easy & medium & hard & easy & medium & hard \\
\midrule
Devstral & N_2, R, N, P, (V, N)^2 & (N, R)^2, N, P, V, N & (N_3, R_2)^2, N, P, (V, N)^2 & N_2, R, N, P, V, N, V & N, P, (V, N)^2, V & (N, R)^3, N, P, V \\
GPT5-mini & (N, P)^2, V, P & (N, P)^3, V & (N_4, P)^5, V, P & (N, P)^3, V & (N, P)^3, V & (N, P)^4 \\
Deepseek-V3 & N, P, V & R_2, N, P, V & N_2, P, V_4 & (P, V)^2 & (P, V)^2 & (P, V)^2 \\
Deepseek-R1 & N, P, V & N, P, V & R_2, N_2, P_4 & N, P, V & N, P, V, P & (N, P)^2 \\
\bottomrule
\end{tabularx}
% \textcolor{blue}{MH: It would be better to use all four phases (N,R,P,V) here instead of combining (N,R) into L.}
\caption{Top $\mathcal{LCP}$s of studied models, conditioned on repair status and problem difficulty. 
% Phases: L=\colorbox[HTML]{D4CCE6}{Localization}, P=\colorbox[HTML]{FFE18E}{Patching}, V=\colorbox[HTML]{D4E7CD}{Validation}. 
Superscripts denote pattern repetition and subscripts denote phase duration (run-length from \lang). \jatin{I would move this to Appendix and use the space to make Fig. 5 larger. Same with Table 4 to make space for FIg. 8. Tables 3 and 4 can be easily integrated into Table 5 as additional rows}}
\label{tab:plan_lcp}
\end{table*}

==> tables/plan_success_rate.tex <==
\begin{table}[t]
% \vspace{-1cm}
\caption{Model Performance Comparison by Difficulty Level}
\centering
\label{tab:plan_perf}
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Easy} & \textbf{Medium} & \textbf{Hard} & \textbf{Overall} \\
\midrule
GPT5-mini & 69 & 53 & 19 & 56 \\
Deepseek-V3 & 53 & 32 & 7 & 38 \\
Devstral-small & \textbf{80} & \textbf{60} & \textbf{24} & \textbf{64} \\
Deepseek-R1 & 53 & 25 & 5 & 39 \\
\bottomrule
\end{tabular}

% \vspace{-1cm}
\end{table}

==> tables/step_added_lcp.tex <==
\makeatletter
\newcommand{\pat}[1]{%
  \begingroup\mathsurround=0pt
  \catcode`\,=\active \catcode`\(=\active \catcode`\)=\active
  \def,{\mskip\thinmuskip\allowbreak,\mskip\thinmuskip}%
  \def({\mskip\thinmuskip(\allowbreak}%
  \def){\allowbreak)\mskip\thinmuskip}%
  \ensuremath{\langle #1 \rangle}%
  \endgroup
}
\makeatother
% Compact but readable table spacing
\newcolumntype{Z}{>{\raggedright\arraybackslash}X}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.06}

\begin{table*}[t]
\centering
\tiny
% %\vspace{-10pt}
\begin{tabularx}{\textwidth}{ll @{\extracolsep{\fill}} ccc ccc }
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Settings}} & \multicolumn{3}{c}{\textbf{Resolved}} & \multicolumn{3}{c}{\textbf{Unresolved}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
& & easy & medium & hard & easy & medium & hard \\
\midrule
\multirow{4}{*}{Devstral} & Regression & $P, (V, N)^3, V$ & $(N, R)^3, N, P, V$ & $P, (V, N)^3, V$ & $(V, N)^3, V$ & $(P, (V, N)^3, V$ & $(V, P)^4, V$ \\
 & Summary & $N_2, R, N, P, V, N, V$ & $(N_2, R)^3, N, P$ & $((N_4, R_2)^2, N, P, (V, N)^2$ & $N_2, R, N, P, V, N, V$ & $(N, R)^2, N, P, V$ & $N, (P, V)^3$ \\
 & Reordered & $P, (V, N)^3, V$ & $(N_2, R)^2, N, P, V, N$ & $(P, N)^2, P, V, N, (P, V)^2$ & $(N_4, R)^3, N$ & $P, (V, N)^3$ & $(N, R)^3, N, P$ \\
 & Reminded & $P, (V, N)^3, V$ & $N_2, R, N, P, (V, N)^2$ & $(N_4, R)^3, N, P, V$ & $(P, (V, N)^3, $ & $(N_2, R)^2, N, P, V, N$ & $(N, R)^2, N, P, V, N$ \\
\midrule
\multirow{4}{*}{GPT5-mini} & Regression & $(N, P)^3$ & $(N, P)^3$ & $P, N, (P, V)^2, P$ & $(N, P)^3, V$ & $(N, P)^3, V$ & $(N, P)^4$ \\
 & Summary & $(N, P)^2, V, P$ & $(N, P)^3, V$ & $P, V, P, N, (P, V)^2$ & $(N_2, P)^2, V, P$ & $(N_2, P)^2, V, P, V$ & $(P, N)^3, P, V$ \\
 & Reordered & $(N, P)^3$ & $(N, P)^3$ & $(N_5, P)^3, N$ & $(N, P)^3$ & $(N, P)^3, V$ & $(N, P)^4$ \\
 & Reminded & $(N, P)^2, V$ & $(N, P)^3, V$ & $(N_3, P)^3, N$ & $(N_2, P)^3$ & $(N, P)^3, V$ & $(N_2, P)^4, V$ \\
\midrule
\multirow{4}{*}{Deepseek-V3} & Regression & $N, P, V$ & $N, P, V$ & $R_12, N_2, P, V_2, N, V_2, P$ & $(P, V)^2$ & $(P, V)^2$ & $N, P, V$ \\
 & Summary & $N, P, V, P$ & $N, P, V, P$ & $R_7, (P, V)^2, P$ & $N, P, V, P$ & $N, P, V, P$ & $(P, V)^2, P$ \\
 & Reordered & $N, P, V$ & $N, P, V$ & $N_2, P$ & $N, P, V$ & $N, P, V$ & $N, P, V$ \\
 & Reminded & $N, P, V$ & $N, P, V$ & $(P_4, N)^4, P$ & $R, N, P, V$ & $N, P, V$ & $N, P, V, P$ \\
\midrule
\multirow{4}{*}{Deepseek-R1} & Regression & $N, P, V$ & $N_2, P, N$ & $N$ & $N$ & $N$ & $N$ \\
 & Summary & $N, P$ & $P, V_3$ & $N_2, P_2$ & $N$ & $N$ & $N$ \\
 & Reordered & $N, P$ & $N, P, V_2$ & $N_2, P$ & $N$ & $N$ & $N, P, V$ \\
 & Reminded & $N, P$ & $N, P$ & $N_2, P, V_3, P$ & $N$ & $N$ & $N$ \\
\bottomrule
\end{tabularx}
\caption{Step added Top $\mathcal{LCP}$s of studied models, conditioned on repair status and problem difficulty. Superscripts denote pattern repetition and subscripts denote phase duration (run-length from \lang).}
\label{tab:stepadded_lcp}
\end{table*}

==> tables/step_removal_lcp.tex <==
\makeatletter
\newcommand{\pat}[1]{%
  \begingroup\mathsurround=0pt
  \catcode`\,=\active \catcode`\(=\active \catcode`\)=\active
  \def,{\mskip\thinmuskip\allowbreak,\mskip\thinmuskip}%
  \def({\mskip\thinmuskip(\allowbreak}%
  \def){\allowbreak)\mskip\thinmuskip}%
  \ensuremath{\langle #1 \rangle}%
  \endgroup
}
\makeatother
% Compact but readable table spacing
\newcolumntype{Z}{>{\raggedright\arraybackslash}X}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.06}

\begin{table*}[t]
\centering
\tiny
% %\vspace{-10pt}
\begin{tabularx}{\textwidth}{ll @{\extracolsep{\fill}} ccc ccc }
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Settings}} & \multicolumn{3}{c}{\textbf{Resolved}} & \multicolumn{3}{c}{\textbf{Unresolved}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
& & easy & medium & hard & easy & medium & hard \\
\midrule
\multirow{3}{*}{Devstral} & No Val. \& Repr. & $(N, R)^3$ & $(N, R)^3, N$ & $(N_2, R_2)^4$ & $(N, R)^3, N$ & $(N, R)^4$ & $(N, R)^4$ \\
 & No Repr. & $N_2, P, V, N$ & $N, (P, V)^2$ & $(R_5, N)^3, (P_2, V_4, N, V)^2, (N_4, V_7)^4, P, V_5$ & $N_2, P, V, P$ & $(P, V)^2$ & $(N_2, P)^2, V$ \\
 & No Val. & $N, R, N, P, V, N$ & $N, R, N, P, V, N, V$ & $(N_3, R_2)^3, N, P$ & $(N, R)^3, N$ & $(N, R)^3, N$ & $(N, R)^4, N$ \\
\midrule
\multirow{3}{*}{GPT5-mini} & No Val. \& Repr. & $(N, P)^3$ & $(N, P)^3, V$ & $R, (N_3, P_3)^3, V_4, N, P, (V, N_3)^2, (P, N_2)^2, (V_4, P)^2$ & $(N, P)^3, V$ & $(N, P)^3, V$ & $(N, P)^4$ \\
 & No Repr. & $(N, P)^2, V$ & $(N, P)^3, V$ & $(N, P)^3, N, V, P, V$ & $(N, P)^3, V$ & $(N, P)^3, V$ & $(N, P)^5$ \\
 & No Val. & $(N_2, P)^3$ & $(N, P)^2, V$ & $(N_2, P)^3, V, P, V_2$ & $(N, P)^3, V$ & $(N, P)^3, V$ & $(N, P)^3, V$ \\
\midrule
\multirow{3}{*}{Deepseek-V3} & No Val. \& Repr. & $N, P$ & $N, P$ & $P$ & $N, P$ & $N, P$ & $N_2, P$ \\
 & No Repr. & $N, P$ & $N, P$ & $P$ & $N, P$ & $N, P$ & $N, P$ \\
 & No Val. & $N, P, V$ & $N, P, V$ & $N_3, P$ & $N, P, V$ & $N, P, V$ & $N, P, V$ \\
\midrule
\multirow{3}{*}{Deepseek-R1} & No Val. \& Repr. & $N, P$ & $(N, P)^2$ & $N_5, P$ & $N$ & $N$ & $N, P$ \\
 & No Repr. & $N, P$ & $N, P, V$ & $P$ & $N, P$ & $N, P$ & $N, P$ \\
 & No Val. & $N, P$ & $N, P$ & $N_2, P$ & $N$ & $N$ & $N$ \\
\bottomrule
\end{tabularx}
\caption{Step removal Top $\mathcal{LCP}$s of studied models, conditioned on repair status and problem difficulty. Superscripts denote pattern repetition and subscripts denote phase duration (run-length from \lang).}
\label{tab:stepremoval_lcp}
\end{table*}
